On the Instrumental Discrepancies in Lyman-alpha Observations of Solar Flares

Despite the energetic significance of Lyman-alpha (Ly{\alpha}; 1216\AA) emission from solar flares, regular observations of flare related Ly{\alpha} have been relatively scarce until recently. Advances in instrumental capabilities and a shift in focus over previous Solar Cycles mean it is now routinely possible to take regular co-observations of Ly{\alpha} emission in solar flares. Thus, it is valuable to examine how the instruments selected for flare observations may influence the conclusions drawn from the analysis of their unique measurements. Here, we examine three M-class flares each observed in Ly{\alpha} by GOES-14/EUVS-E, GOES-15/EUVS-E, or GOES-16/EXIS-EUVS-B, and at least one other instrument from PROBA2/LYRA, MAVEN/EUVM, ASO-S/LST-SDI, and SDO/EVE-MEGS-P. For each flare, the relative and excess flux, contrast, total energy, and timings of the Ly{\alpha} emission were compared between instruments. It was found that while the discrepancies in measurements of the relative flux between instruments may be considered minimal, the calculated contrasts, excess fluxes, and energetics may differ significantly - in some cases up to a factor of five. This may have a notable impact on multi instrument investigations of the variable Ly{\alpha} emission in solar flares and estimates of the contribution of Ly{\alpha} to the radiated energy budget of the chromosphere. The findings presented in this study will act as a guide for the interpretation of observations of flare-related Ly{\alpha} from upcoming instruments during future Solar Cycles and inform conclusions drawn from multi-instrument studies.

==> commands.tex <==
% Please use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared
\newcommand\todo[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\corot}{{\it CoRoT}}
\newcommand{\tess}{{\it TESS}}
\newcommand{\plato}{{\it PLATO}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\JWST}{{\it JWST}}
\newcommand{\NGTS}{NGTS}
\newcommand{\TESS}{{\it TESS}}
\newcommand{\gpe}{{GP-EBOP}}
\newcommand{\LSO}{La Silla Observatory}
\newcommand{\PAR}{Paranal Observatory}
\newcommand{\etop}{\emph{top}}
\newcommand{\emid}{\emph{middle}}
\newcommand{\ebot}{\emph{bottom}}
\newcommand{\eleft}{\emph{left}}
\newcommand{\eright}{\emph{right}}
\newcommand{\eTop}{\emph{Top}}
\newcommand{\eMid}{\emph{Middle}}
\newcommand{\eBot}{\emph{Bottom}}
\newcommand{\eLeft}{\emph{Left}}
\newcommand{\eRight}{\emph{Right}}
\newcommand{\btgc}[1]{\textcolor{blue}{[BTG: #1]}}
\newcommand{\jsj}[1]{\textcolor{blue}{[JSJ: #1]}}
% UNITS
\newcommand{\kms}{km\,s$^{-1}$}
\newcommand{\ms}{m\,s$^{-1}$}
\newcommand{\masy}{mas\,y$^{-1}$}
\newcommand{\mpl}{\mbox{M$_{P}$}}
\newcommand{\rpl}{\mbox{R$_{P}$}}
\newcommand{\rhopl}{\mbox{$\rho_{P}$}}
\newcommand{\mstar}{\mbox{M$_{*}$}}
\newcommand{\rstar}{\mbox{R$_{*}$}}
\newcommand{\rhostar}{\mbox{$\rho_{*}$}}
\newcommand{\mjup}{\mbox{M$_{J}$}}
\newcommand{\rjup}{\mbox{R$_{J}$}}
\newcommand{\rhojup}{\mbox{$\rho_{J}$}}
\newcommand{\mearth}{\mbox{M$_{\oplus}$}}
\newcommand{\rearth}{\mbox{R$_{\oplus}$}}
\newcommand{\msun}{\mbox{M$_{\odot}$}}
\newcommand{\rsun}{\mbox{R$_{\odot}$}}
\newcommand{\gccc}{g\,cm$^{-3}$}
\newcommand{\ergscm}{erg\,s$^{-1}$cm$^{-2}$}
\newcommand{\teff}{$T_{\rm eff}$}
\newcommand{\feh}{\mbox{[Fe/H]}}
\newcommand{\vsini}{\mbox{$v\sin i$}}
\newcommand{\logg}{$\log g$}
\newcommand{\tc}{$T_C$}
\newcommand{\rprs}{\mbox{R$_{P}/$R$_{*}$}}
\newcommand{\lya}{Ly$\rm \alpha$}
\newcommand{\ergs}{erg\,s$\rm ^{-1}$}
\newcommand{\ec}{E$\rm _{c}$}
%Maths stuff
\newcommand{\lnL}{\mbox{$\ln\mathcal{L}$}}
\newcommand{\scin}{scintillation}
\newcommand{\sigY}{$\sigma_{\scriptscriptstyle \text{Y}}$}
\newcommand{\sigYmath}{\sigma_{\scriptscriptstyle \text{Y}}}
\newcommand{\Cy}{$C_{\scriptscriptstyle \text{Y}}$}
\newcommand{\CyMath}{C_{\scriptscriptstyle \text{Y}}}
\newcommand{\Gmag}{$G_{\text{mag}}$}

==> references.tex <==
% This file is required for arXiv submission.

